MentalManip: A Dataset For Fine-grained Analysis of Mental Manipulation in Conversations

Mental manipulation, a significant form of abuse in interpersonal conversations, presents a challenge to identify due to its context-dependent and often subtle nature. The detection of manipulative language is essential for protecting potential victims, yet the field of Natural Language Processing (NLP) currently faces a scarcity of resources and research on this topic. Our study addresses this gap by introducing a new dataset, named ${\rm M{\small ental}M{\small anip}}$, which consists of $4,000$ annotated movie dialogues. This dataset enables a comprehensive analysis of mental manipulation, pinpointing both the techniques utilized for manipulation and the vulnerabilities targeted in victims. Our research further explores the effectiveness of leading-edge models in recognizing manipulative dialogue and its components through a series of experiments with various configurations. The results demonstrate that these models inadequately identify and categorize manipulative content. Attempts to improve their performance by fine-tuning with existing datasets on mental health and toxicity have not overcome these limitations. We anticipate that ${\rm M{\small ental}M{\small anip}}$ will stimulate further research, leading to progress in both understanding and mitigating the impact of mental manipulation in conversations.

==> tables/taxonomy.tex <==
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}

\begin{table}[t!]
\centering
\small
\caption{Multi-level annotation taxonomy.}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{c|l|l}
\hline
\textbf{\makecell{Presence of\\Manipulation}} & \textbf{\makecell{Manipulation\\Technique}} & \textbf{\makecell{Targeted\\Vulnerability}}\\ 
\hline
\multicolumn{1}{c|}{\multirow{12}{*}{Manipulative}} & \makecell{1. Denial or Minimization}  & 1. Over-responsibility
\\  
\multicolumn{1}{c|}{} & 2. Rationalization  & 
\\  
\multicolumn{1}{c|}{} & 3. Feigning innocence & 2. Overthinking
\\  
\multicolumn{1}{c|}{} & 4. Feigning confusion  & 
\\  
\multicolumn{1}{c|}{} & 5. Intimidation & 3. Naivete
\\  
\multicolumn{1}{c|}{} & 6. Shaming  & 
\\  
\multicolumn{1}{c|}{} & 7. Accusation & 4. Low self-esteem 
\\   
\multicolumn{1}{c|}{} & 8. Ignorance  & 
\\   
\multicolumn{1}{c|}{} & 9. Playing the victim  &  5. Dependency 
\\   
\multicolumn{1}{c|}{} & 10. Playing the servant   & 
\\   
\multicolumn{1}{c|}{} & 11. Seduction & 
\\   
\multicolumn{1}{c|}{} & 12. Bandwagon effect & 
\\ \hline
\makecell{Non- \\ manipulative} & / & / 
\\ \hline
\end{tabular}
% }
\label{table:taxonomy}
\end{table}
